Hybrid multi-observer for improving estimation performance

Various methods are nowadays available to design observers for broad classes of systems, where the primary focus is on establishing the convergence of the estimated states. Nevertheless, the question of the tuning of the observer to achieve satisfactory estimation performance remains largely open. In this context, we present a general design framework for the online tuning of the observer gains. Our starting point is a robust nominal observer designed for a general nonlinear system, for which an input-to-state stability property can be established. Our goal is then to improve the performance of this nominal observer. We present for this purpose a new hybrid multi-observer scheme, whose great flexibility can be exploited to enforce various desirable properties, e.g., fast convergence and good sensitivity to measurement noise. We prove that an input-to-state stability property also holds for the proposed scheme and, importantly, we ensure that the estimation performance in terms of a quadratic cost is (strictly) improved. We illustrate the efficiency of the approach in improving the performance of given nominal observers in two numerical examples (Van der Pol oscillator and Lithium-Ion (Li-Ion) battery model).

==> commands-letter.tex <==


\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Rl}[2]{\ensuremath{\mathbb{R}^{#1}_{#2}}}   % Euclidean space
\newcommand{\Rlp}{\ensuremath{\mathbb{R}_{>0}}}
\newcommand{\Rlo}{\ensuremath{\mathbb{R}_{\geq 0}}}
\newcommand{\Zo}{\ensuremath{\mathbb{Z}_{\geq 0}}}
\newcommand{\Zp}{\ensuremath{\mathbb{Z}_{> 0}}}
\newcommand{\C}[1]{\ensuremath{\mathbb{C}^{#1}}}         % Complex plane
\newcommand{\N}{\ensuremath{\mathbb{N}}}                 % Set of natural numbers
\newcommand{\No}{\ensuremath{\mathbb{N}_{0}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}

\DeclareMathOperator*{\argmin}{argmin}


\newcommand\blue[1]{{\color{blue}#1}}

\newcommand{\Linf}[1]{\ensuremath{\mathcal{L}^{#1}}}

\newcommand{\eg}{{\it e.g., }}


\newcommand{\KL}{\ensuremath{\mathcal{KL}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\Kinf}{\ensuremath{\mathcal{K}_{\infty}}}
\newcommand{\KK}{\ensuremath{\mathcal{KK}}}
\newcommand{\KKL}{\ensuremath{\mathcal{KKL}}}
\newcommand{\KLL}{\ensuremath{\mathcal{KLL}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}

% Flow and jump sets
\newcommand{\Cs}{\ensuremath{C_{\text{steady}}}}
\newcommand{\Ct}{\ensuremath{C_{\text{transient}}}}
\newcommand{\Ds}{\ensuremath{D_{\text{steady}}}}
\newcommand{\Dt}{\ensuremath{D_{\text{transient}}}}

%\newcommand{\d}{\ensuremath{\delta}}

\newcommand{\interior}{\ensuremath{\text{int}\,}}

\newcommand{\dom}{\ensuremath{\text{dom}\,}}
\newcommand{\ext}{\ensuremath{\text{ext}}}
\newcommand{\rge}{\ensuremath{\text{rge}\,}}
\newcommand{\diag}{\ensuremath{\text{diag}\,}}
\newcommand{\esup}{\ensuremath{\text{ess.sup}\,}}


\newcommand{\sign}[1]{\ensuremath{\text{sign}{(#1)}}}
\newcommand{\sat}{\ensuremath{\text{sat}}}

\newcommand{\sinc}{\ensuremath{\text{sinc}}}
\newcommand{\nom}{\ensuremath{\text{nom}}}


\newcommand{\Tmati}{\ensuremath{T_{MATI}\,\,}}
\newcommand{\Tmasp}{\ensuremath{\mathrm{T_{MASP}}\,}}
\newcommand{\lc}{\ensuremath{\llbracket}}
\newcommand{\rc}{\ensuremath{\rrbracket}}
%\newcommand{\arg}{\ensuremath{\text{arg}}}
%

\newcommand{\norm}[1]{\ensuremath{\left\|{#1}\right\|}}
\newcommand{\ip}[2]{\ensuremath{\left\langle #1, #2\right\rangle}}
\newcommand{\cb}[1]{\ensuremath{\overline{\mathbb{B}}_{\mbox{\scriptsize $#1$}}}}                              % Closed unit ball
\newcommand{\ob}[2]{\ensuremath{\mathbb{B}_{\mbox{\scriptsize $#1$}}\ensuremath{\left( #2\right)}}}   % Open unit ball
\newcommand{\df}{\ensuremath{\stackrel{\mbox{\tiny $\mathrm{def}$}}{=}\:}}                                             % Defined by
\newcommand{\myint}[4]{\ensuremath{\int_{#1}^{#2}#3\;\mathrm{d}#4}}
\newcommand{\Mm}{\ensuremath{\:\stackrel{\rightarrow}{\scriptstyle{\rightarrow}}\:}}
%\newcommand{\bm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\hs}[1]{\hspace*{#1 em}}
%\newcommand{\summ}{\ensuremath{\sum_{i\in\mathcal{I}}}}
\newcommand{\qa}{\ensuremath{\mathcal{Q}_{A}}}%
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\di}{\ensuremath{\mathcal{D}_{i}}}


%
%\newcounter{eq}
%\newcommand{\arabalph}{\stepcounter{equation}%
%\setcounter{eq}{\value{equation}}%
%\setcounter{equation}{0}%
%\renewcommand{\theequation}{\theeq\alph{equation}}}
%\newcommand{\arab}{\setcounter{equation}{\value{eq}}%
%\renewcommand{\theequation}{\arabic{equation}}}

%\newtheoremstyle{note}% name
%  {3pt}%      Space above
%  {3pt}%      Space below
%  {}%         Body font
%  {}%         Indent amount (empty = no indent, \parindent = para indent)
%  {\itshape}% Thm head font
%  {:}%        Punctuation after thm head
%  {.5em}%     Space after thm head: " " = normal interword space;
%        %       \newline = linebreak
%  {}%         Thm head spec (can be left empty, meaning `normal')
%
%\theoremstyle{note}
%\newtheorem{note}{Note}


% Commandes d'Adolfo
\newcommand{\ie}{{\it i.e. }}

\newtheorem{exple}{Example}
\newtheorem{defn}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{hypo}{Hypothesis}
\newtheorem{ass}{Assumption}
%\newtheorem*{sass*}{Standing Assumption}
\newtheorem{prop}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{lem}{Lemma}
\newtheorem{ex}{Example}
\newtheorem{thm}{Theorem}
\newtheorem{cor}{Corollary}
\newtheorem{pb}{Problem}
%\newtheorem{proof}{Proof}[section]
\newtheorem{rem}{Remark}


%\newtheorem{exple}{Example}[section]
%\newtheorem{defn}{Definition}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{hypo}{Hypothesis}[section]
%\newtheorem{ass}{Assumption}[section]
%\newtheorem{prop}{Proposition}[section]
%\newtheorem{fact}{Fact}[section]
%\newtheorem{lem}{Lemma}[section]
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{cor}{Corollary}[section]
%%\newtheorem{proof}{Proof}[section]
%\newtheorem{rem}{Remark}[section]



%
%  Remark environment
%
%\newenvironment{rem}{\textit{Remark. }}{\mbox{}\\[1ex]}
\newenvironment{rems}{\textit{Remarks. }}{\mbox{}\\[1ex]}
%

% Claudio's commands

%\usepackage[overload]{abraces}

\def\startmodif{\color{blue}}
%\def\startmodif{\color{black}}
\def\stopmodif{\color{black}} %yyy


\def\startmodifg{\color{magenta}}
%\def\startmodif{\color{black}}
\def\stopmodifg{\color{black}} %yyy

\newcommand{\margin}[1]{\marginpar{\tiny\color{blue} #1}}


\newcommand{\ave}{{\rm ave}}
%\newcommand{\degree}{{\rm deg}}
\newcommand{\dst}{\displaystyle}
\newcommand{\Ni}{\mathcal{N}_i}
\newcommand{\Si}{\mathcal{S}_i}
\newcommand{\Ei}{\mathcal{E}_i}

\newtheorem{remark}{Remark}

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\ba{\begin{array}}
\def\ea{\end{array}}




